Computational Cost Reduction in Learned Transform Classifications

We present a theoretical analysis and empirical evaluations of a novel set of techniques for computational cost reduction of classifiers that are based on learned transform and soft-threshold. By modifying optimization procedures for dictionary and classifier training, as well as the resulting dictionary entries, our techniques allow to reduce the bit precision and to replace each floating-point multiplication by a single integer bit shift. We also show how the optimization algorithms in some dictionary training methods can be modified to penalize higher-energy dictionaries. We applied our techniques with the classifier Learning Algorithm for Soft-Thresholding, testing on the datasets used in its original paper. Our results indicate it is feasible to use solely sums and bit shifts of integers to classify at test time with a limited reduction of the classification accuracy. These low power operations are a valuable trade off in FPGA implementations as they increase the classification throughput while decrease both energy consumption and manufacturing cost.

==> my_files/table_mnist_cifar_10_error_and_num_bits_D_X.tex <==
%!TEX root = ../machado_cost_reduction_classifiers_2016.tex
%<*header>
 & \multicolumn{2}{c}{MNIST} & \multicolumn{2}{c}{CIFAR-10} \\ 
\cmidrule(r){2-3} \cmidrule(l){4-5}
 & \multicolumn{1}{c}{Error \%} & \multicolumn{1}{c}{\# bits D'X} & \multicolumn{1}{c}{Error \%} & \multicolumn{1}{c}{\# bits D'X} \\ 
%</header>
%<*data>
Original & 1.71 & 61 & 46.27 & 55 \\ 
Proposed & 2.23 & 34 & 49.92 & 37 \\ 
%</data>

